A bounded-degree network formation game

Motivated by applications in peer-to-peer and overlay networks we define and study the \emph{Bounded Degree Network Formation} (BDNF) game. In an $(n,k)$-BDNF game, we are given $n$ nodes, a bound $k$ on the out-degree of each node, and a weight $w_{vu}$ for each ordered pair $(v,u)$ representing the traffic rate from node $v$ to node $u$. Each node $v$ uses up to $k$ directed links to connect to other nodes with an objective to minimize its average distance, using weights $w_{vu}$, to all other destinations. We study the existence of pure Nash equilibria for $(n,k)$-BDNF games. We show that if the weights are arbitrary, then a pure Nash wiring may not exist. Furthermore, it is NP-hard to determine whether a pure Nash wiring exists for a given $(n,k)$-BDNF instance. A major focus of this paper is on uniform $(n,k)$-BDNF games, in which all weights are 1. We describe how to construct a pure Nash equilibrium wiring given any $n$ and $k$, and establish that in all pure Nash wirings the cost of individual nodes cannot differ by more than a factor of nearly 2, whereas the diameter cannot exceed $O(\sqrt{n \log_k n})$. We also analyze best-response walks on the configuration space defined by the uniform game, and show that starting from any initial configuration, strong connectivity is reached within $\Theta(n^2)$ rounds. Convergence to a pure Nash equilibrium, however, is not guaranteed. We present simulation results that suggest that loop-free best-response walks always exist, but may not be polynomially bounded. We also study a special family of \emph{regular} wirings, the class of Abelian Cayley graphs, in which all nodes imitate the same wiring pattern, and show that if $n$ is sufficiently large no such regular wiring can be a pure Nash equilibrium.

==> stable.tex <==
\section{Stable Wiring}\label{sec:}


\begin{theorem}
For any $n\geq 2$ and any positive $k$, there is a uniform stable
$(n,k)$-wiring.
\end{theorem}
\begin{proof}
The theorem is clearly true for $k = 1$ because the directed
Hamiltonian cycle
  is stable.
We first prove the theorem for $k=2$. As it turns out, this is the
hardest case. By Lemma \ref{Lem:DenseRavi}, there are regular
$(n,2)$-stable wirings
  for $n\leq 5$.
In fact, one can easily show that there are regular $(6,2)$- and
$(7,2)$-stable
  wirings as well.
So, we assume $n \geq  8$.

Let $h$ be the largest integer such that $2^{h} -1 \leq  n$. Let
$t = n - (2^{h}-1)$. We will consider the following cases: (0) $t=
0$, (1) $ t = 1\mod  2$, (2) $t = 0 \mod 4$ and (3) $t =2 \mod
    4$.
Although $t=0$ is implied by $t = 0\mod 4$, we handle it
separately for clearity. With the assumption that $n\geq 8$, we
have $h\geq 3$.

Let us first consider the case when $t = 0$. Let $T_{2,h-1}$ be  a
complete binary tree of height
  $h-1$.
Note that $T_{2,h-1}$ has $2^{h}-1 = n$ node. So we label the
nodes of $T_{2,h-1}$ from $[1:n]$ according to the
  in-order traversal of the tree.
Let $r=1$ be the root. See Figure \ref{fig:stable}. Note that the
root $r$ achieves the ``utopian'' cost, which is as good
   as  it can be obtained even it controls all wiring of the links.
\begin{figure}[htb]
\begin{center}
\includegraphics[width=2.5in]{n2treexfigwish.eps}
\caption{An example of a stable wiring} \label{fig:stable}
\end{center}
\end{figure}
We choose the leftmost leaf, the node with lable $2^{h-1}$,
  and use one of its out-link to connect to the root $r$.
We connect its other outlink to the right children, node 3, of the
  root.
We connect all other leaves directly with 2 and 3, the two
children
  of the root.
We now argue that this wiring is stable. Clearly, the root is
stable, simply because it has an uptopian cost. All internal nodes
are stable for the reason that any rewire
  will disconnect it from the nodes in the subtree it no longer
  connects to.

Consider node $2^{h-1}$. We will call it the bridge node. Rewire
its link to  the root will disconnect it from the root. It
suffices to show that it can not rewire its other outlink. We
first observe that a rewiring to 2 is worse because it will
increase
  the cost of the bridge node by 1:
  its distance to  every node in $T[3]$, the subtree rooted at 3
  increases by 1 and its distance to every node in $T[2]$
  other than itself decreases by 1.
Consider a rewiring of this link to a children of 3, say, its left
  children 6 (recall we assume $n\geq 8$).
Its distances to the root, and to every node in $T[2]$
  remains the same.
Its distances to 3 and to every node in its
  right subtree increase by 1, and its disances to every node in the left
  subtree of 3 decrease by 1.
So the net loss is 1. Recursively, with the same argument, we can
easily show
  that a rewiring to any node in the subtree of 3
  induces a loss.
Similarly, we can show that a rewiring to any nodes in $T[2]$
   is worse than the rewiring to 2 itself.
So, 3 is the best choice of $2^{h-1}$. For other leaves, their
total distance is equal to the utopian + 1. Since no rewiring will
make them utopian, they are stable as well.


To prove the other three cases, the key is to view the wiring
  correctly.
We now discuss our ``correct'' view. Recall $t = n - (2^{h}-1)$.
We will view nodes $[2^{h}:n]$ and 1 all as roots. Note that
$[2^{h}:n] = [n-t+1:n]$. Both $T[2]$ and $T[3]$ are complete
binary tree of height h-2. We connect all these roots to 2 and 3.
All roots are in the state of uptopian. See Figure
\ref{fig:generalStable}.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=3.5in]{n2treeGeneral.eps}
\caption{General stable wiring} \label{fig:generalStable}
\end{center}
\end{figure}

In other words, in Case 0, we have one root. Now we have multiple
roots. Let $L[2]$, $R[2]$, $L[3]$, and $R[3]$,
  respectively denote the subtree of height $h-3$,
  rooted at the children of 2 and 3.

The rule for our wiring is very simple! Case 1, when $t+1 = 0 \mod
2$, is the easiest case. We pair up these roots and suppose we
have $p$ pairs. We can choose any $p$ leaves and
  uses their out-links to connect to these pairs of roots.
The rest of the leaves are connected to 2 and 3. Clearly, all
roots are stable. All leaves that are not connected to roots have
cost utopian +1,
  so they are stable.
All other nodes are ``internal'' and they are stable because any
  rewiring locally will disconnect it from some nodes.

In Case 2, we have $t+1 = 1 \mod  4$. Suppose $t = 4p$. We form
$2p$ pairs of roots with root $n$ unpaired. If $2p \leq 2^{h-3}$,
the number of leaves in $T[2]$,
  we choose $p$ leaves from $L[2]$ and $p$ leaves from $R[2]$
  uses their out-links to connect to these pairs.
If $2p > 2^{h-3}$,  then we choose all leaves in $T[2]$
   and also choose $(2p-2^{h-3})/2$ leaves from $L[3]$ and $R[3]$.
We use their out-links to connect to these pairs of roots.
Finally, we select a not-yet-chosen leaf $v$ from $T[3]$. Without
loss of generality, assume $v = 2^{h}-1$. We refer to it as
  the bridge node.
We use one of its out-link to connect to $n$ and the other link to
  connect to $2$.
The rest of the leaves are connected to 2 and 3. Again, all roots
and all ``internal'' nodes including those
  leaves that are connected to two roots are stable.
All non-bridge leaves have cost utopian+1, so they are stable. As
for the bridge node $v$, its link to $r$ can not be rewired. If $p
= 0$, we have case 0. So $v$ is stable. Otherwise, $p>0$, and the
subtree of $2$ connects to at least $4$ more
  roots than the subtree of $3$.
So for $v$, connecting to $2$ is strictly better than connecting
to
  $3$.
Because $L[2]$ and $R[2]$ connects to the same number of roots,
 it is inferior to rewire the link to other nodes in $T[2]$.
So, $v$ is stable as well.

In Case 3, we have $t+1 = 3 \mod  4$. Suppose $t - 2 = 4p$. We
form $2p$ pairs of roots
  with $1$, $n-1$, and $n$ unpaired.
When $p>0$, we use the same approach of Case 2 to connect to these
  roots.
Then, we select a leaf $v_{1}$ from $L[3]$ and a leaf $v_{2}$ from
$R[3]$. Without loss of generality, assume $v_{2} = 2^{h}-1$. We
refer to it as
  the bridge node.
We connect $v_{1}$ to $1$ and $n-1$ and $v_{2}$ to $r_{3}$. We
also connect $v_{2}$  to $2$. With the same argument as in Case 2,
we can show that
   all nodes are  stable.

The most tricky case is when $p = 0$, i.e., we have three roots.
So far, we have only found one family of stable solutions to this
case. See Figure \ref{fig:general3Root}. Other than the three
bridge nodes, all other leaves connects to 2 and 3.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=3.5in]{n2tree3Root.eps}
\caption{Case with three roots} \label{fig:general3Root}
\end{center}
\end{figure}
With the same argument, we can prove that all non-bridge nodes are
  stable.
As bridge nodes $u$ and $v$ are symmetric,
  we will only prove $u$ is stable.
Clearly, it can not rewire its link to 1. Because $T[2]$ connects
to one more root
  than $T[3]$, and $u$ belong to $L[2]$,
  the wiring $(u,2)$ and $(u,3)$ induces the same cost for $u$.
If $u$ is connected to $2$, our earlier argument will show
  moving the link down the tree can only increase the cost.
If $u$ is connected to $3$, because the number of
  roots connected by $L[3]$ is one less than the numbers of roots
  connected by $R[3]$, connecting $u$ to the root of $L[3]$
  also increases the distance to 3 by 1.
So rewiring to the root of $L[3]$ is worse than connecting
  to $3$.
With a similar calculation, connecting to the root of $R[3]$
induces the
  sames cost as connecting to $3$.
Inductively, we can show $(u,3)$ is as good as any other
connection. So, $u$ is stable. Similarly, we can show $w$ is
stable.

This completes the proof for $k = 2$. For $k \geq 3$, the proof is
similar. The basic idea is start with the largest
  complete $k$-nary tree that has no more than $n$ nodes.
Suppose the height of this tree is $h$. So this tree has $n_{k,h}
= \sum_{i=0}^{h} k^{i}$ nodes. Let $t = n - n_{k,h}$. We also call
other $t$ nodes roots and connect them to
  the $k$ children of 1, i.e., $[2:k+1]$.
Let $t_{1} = t \mod k$. We group $t-t_{1}$ roots into tuples, each
has k roots.

We use the subtrees rooted at  first two children of 2
  to evenly connect these tuples.
These two subtrees played the role of $L[2]$ and $R[2]$
  in our proof for $k=2$.
If the number of the tuples is odd, we connect to root in
  one of the tuple from  a leaf not in these two subtrees.
If these two trees are full, we uses the leaves from left to right
to
  connect to roots.

We use the rightmost leaf  of the subtree rooted at $k+1$
  as our bridge node.
The bridge node connects to $t_{1}$ roots. Other links of the
bridge nodes connects to nodes in $[2:k+1]$
  in the order of the number of leaves that their subtrees connect to.
All other leaves connects to $[2:k+1]$

Similar to the case when $k=2$, we can prove all nodes are stable.
In fact, the argument is easier, because moving a link down the
  tree loses more when $k>2$.
\end{proof}

